Teichm\"uller spaces and bounded symmetric domains do not mix isometrically

This paper shows that, in dimensions two or more, there are no holomorphic isometries between Teichm\"uller spaces and bounded symmetric domains in their intrinsic Kobayashi metrics.

==> bibliography.tex <==
% ----------------------------------------------------------------

\let\oldthebibliography=\thebibliography
\let\endoldthebibliography=\endthebibliography
\renewenvironment{thebibliography}[1]
  {
    \begin{oldthebibliography}{#1}
    \setlength{\itemsep}{1ex}
  }
  {
    \end{oldthebibliography}
  }

% ----------------------------------------------------------------
%   MOVE THE TWO BIBLIOGRAPHY FILES IN THE LOCAL FOLDER BEFORE 
%                  CREATING THE FINAL TARBALL
% ----------------------------------------------------------------

\bibliographystyle{math}
\bibliography{math}

% ----------------------------------------------------------------

%%% Local Variables:
%%% TeX-master: "main"
%%% End:

% ----------------------------------------------------------------
